The Power of Menus in Contract Design

We study the power of menus of contracts in principal-agent problems with adverse selection (agents can be one of several types) and moral hazard (we cannot observe agent actions directly). For principal-agent problems with $T$ types and $n$ actions, we show that the best menu of contracts can obtain a factor $\Omega(\max(n, \log T))$ more utility for the principal than the best individual contract, partially resolving an open question of Guruganesh et al. (2021). We then turn our attention to randomized menus of linear contracts, where we likewise show that randomized linear menus can be $\Omega(T)$ better than the best single linear contract. As a corollary, we show this implies an analogous gap between deterministic menus of (general) contracts and randomized menus of contracts (as introduced by Castiglioni et al. (2022)).

==> header.tex <==
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{bbm}
\usepackage{bm}
\usepackage{booktabs}
\usepackage{cleveref}
\usepackage{enumitem}
\usepackage{graphicx}
\usepackage{mathtools}
\usepackage{multirow}
\usepackage{nicefrac}
\usepackage{subcaption}
\usepackage{thm-restate}
\usepackage{tikz}
\usetikzlibrary{calc}
\usepackage{fullpage}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage{wrapfig}
\usepackage{xspace}
\usepackage{csquotes}

\newtheorem{theorem}{Theorem}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{problem}{Open Problem}
\newtheorem{question}{Question}

\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}

% Author Comment Macros
%\newcommand{\jonnote}[1]{{\color{green}{(Jon: #1)}}}
%\newcommand{\joshnote}[1]{{\color{red}{Josh: #1}}}
%\newcommand{\ggnote}[1]{{\color{blue}{Guru: #1}}}
%\newcommand{\junyaonote}[1]{{\color{magenta}{Junyao: #1}}}

\newcommand{\jonnote}[1]{}
\newcommand{\joshnote}[1]{}
\newcommand{\ggnote}[1]{}
\newcommand{\junyaonote}[1]{}

% Math Macros
\newcommand{\indicator}[1]{\mathcal{I}\left(#1\right)}
\newcommand{\D}{\mathcal{D}}
\newcommand{\B}{\mathcal{B}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\eps}{\varepsilon}
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}

% Puts a bar underneath a symbol.
\newcommand{\ubar}[1]{\text{\b{$#1$}}}

\def \Rev  {{\sf Rev}}
\def \Welf  {{\sf Welf}}

\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}
\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
\DeclarePairedDelimiter{\norm}{\|}{\|}
\DeclarePairedDelimiter{\braket}{ \left \langle}{ \right \rangle}
\DeclarePairedDelimiter{\set}{ \{ }{ \} }
\newcommand{\bkt}[2]{\braket{#1, #2}}


\newcommand{\dist}[3]{d_{#3}\left(#1, #2\right)}


\newcommand{\I}{\ensuremath{\mathcal{I}}}
\newcommand{\poly}{\mathrm{poly}}

\newcommand{\Derivative}[1]{\frac{d}{d#1}}

\newcommand{\DSet}{\textnormal{Dominating-Set}\xspace}


\newcommand{\InstMenu}{\textsc{Optimal-Menu}\xspace}
\newcommand{\InstContract}{\textsc{Optimal-Contract}\xspace}

% Principal-Agent Problem Macros
  % Cost, Obsolete
  \newcommand{\cost}[1]{c_{#1}}
  \newcommand{\costvector}{\bm{c}}
  % Cost
  \newcommand{\Cost}[1]{c_{#1}}
  \newcommand{\CostVector}{\bm{c}}
  \newcommand{\TypedCostVector}[1]{\bm{c}^{(#1)}}
  
  % Forecast
  \newcommand{\Forecast}[2]{F_{#1, #2}}
  \newcommand{\TypedForecast}[3]{F^{(#1)}_{#2, #3}}
  \newcommand{\ForecastMatrix}{F}
  \newcommand{\TypedForecastMatrix}[1]{F^{(#1)}}
  \newcommand{\ForecastTensor}{\bm{F}}
  
  % Reward, Obsolete
  \newcommand{\reward}[1]{r_{#1}}
  \newcommand{\rewardvector}{\bm{r}}
  % Reward
  \newcommand{\Reward}[1]{r_{#1}}
  \newcommand{\RewardVector}{\bm{r}}
  
  % Expected Reward
  \newcommand{\TypedExpectedReward}[2]{R^{(#1)}_{#2}}
  \newcommand{\ExpectedReward}[1]{R_{#1}}
  
  % Overall Principal-Agent Problem
  \newcommand{\PrincipalAgentProblem}{\left(\costvector, \ForecastTensor, \rewardvector\right)}
  \newcommand{\PrincipalAgentProblemPrime}{\left(\costvector', \ForecastTensor', \rewardvector'\right)}
  
  % Contract
  \newcommand{\Contract}[1]{x_{#1}}
  \newcommand{\TypedContract}[2]{x^{(#1)}_{#2}}
  \newcommand{\ContractVector}{\bm{x}}
  \newcommand{\TypedContractVector}[1]{\bm{x}^{(#1)}}
  \newcommand{\TypedContractPrime}[2]{x^{\prime(#1)}_{#2}}
  \newcommand{\TypedContractVectorPrime}[1]{\bm{x}^{\prime(#1)}}
  \newcommand{\ContractMatrix}{X}
  \newcommand{\ContractMatrixPrime}{X'}
  \newcommand{\ContractDistributions}{\mathcal{X}}

  % Linear Contracts
  \newcommand{\TransferCoefficient}{\alpha}
  \newcommand{\RLC}{Randomized Linear Contract\xspace}

  % Optimal Action
  \newcommand{\OptimalAction}{i_*}
  \newcommand{\TypedOptimalAction}[1]{\OptimalAction^{(#1)}}

  % Profit
  \newcommand{\Profit}{\textsc{Profit}}
  \newcommand{\TypedProfit}[1]{\Profit^{(#1)}}
  % Utility
  \newcommand{\Utility}{U}

  % Obsolete Macros, replace
  \newcommand{\forecastprime}[3]{F^{\prime(#1)}_{#2, #3}}
  \newcommand{\contract}[1]{x_{#1}}

% Measure Macros
\newcommand{\Measure}{B}
\newcommand{\OWelfare}{\textsc{Welfare}}
\newcommand{\OTypeAware}{\textsc{Opt-TypeAware}}
\newcommand{\ODetMenu}{\textsc{Opt-DetMenu}}
\newcommand{\ORndMenu}{\textsc{Opt-RndMenu}}
\newcommand{\ORndMenuLinear}{\textsc{Opt-RndMenuLinear}}
\newcommand{\OSingle}{\textsc{Opt-Single}}
\newcommand{\OLinear}{\textsc{Opt-Linear}}
\newcommand{\Revenue}{\textsc{Revenue}}

% Linear Algebra Macros
\newcommand{\StandardBasisVector}[1]{\vec{e}_{#1}}

% Complexity Macros
\newcommand{\ApxHard}{\textsc{APX}-Hard\xspace}
\newcommand{\NPHard}{\textsc{NP}-Hard\xspace}

% Accent Macros
\newcommand{\dutting}{D{\"u}tting}
\newcommand{\naive}{na{\"i}ve}
\newcommand{\Naively}{Na{\"i}vely}

% apx-stability.tex
\newcommand{\actionmapping}{(i_1, i_2, \ldots, i_T)}
\newcommand{\optactionmapping}{(i^*_1, i^*_2, \ldots, i^*_T)}

% computation.tex
\newcommand{\neighbor}[2]{\delta_{#1}\left(#2\right)}

\allowdisplaybreaks

==> table-example.tex <==
\begin{table}
\centering
\begin{tabular}{cccccc}
  \toprule
  % Choose a Set Cover
  \multirow{2}{*}{Type $t \in [N]$} & \textbf{Outcome} $1$ & \multirow{2}{*}{$\cdots$} & \textbf{Outcome} $j \in [N]$ & \multirow{2}{*}{$\cdots$} & \textbf{Outcome} $N+1$ \\
                                    & Reward $1$           &                           & Reward $1$                   &                           & Reward $0$             \\ \midrule
  \textbf{Action} $1$ & \multirow{2}{*}{$\indicator{\neighbor{1}{t} = 1}$} & \multirow{2}{*}{$\cdots$} & \multirow{2}{*}{$\indicator{\neighbor{1}{t} = j}$} & \multirow{2}{*}{$\cdots$} & \multirow{2}{*}{$0$} \\ Cost $\tfrac12$ \\
  \textbf{Action} $2$ & \multirow{2}{*}{$\indicator{\neighbor{2}{t} = 1}$} & \multirow{2}{*}{$\cdots$} & \multirow{2}{*}{$\indicator{\neighbor{2}{t} = j}$} & \multirow{2}{*}{$\cdots$} & \multirow{2}{*}{$0$} \\ Cost $\tfrac12$ \\
  \textbf{Action} $3$ & \multirow{2}{*}{$\indicator{\neighbor{3}{t} = 1}$} & \multirow{2}{*}{$\cdots$} & \multirow{2}{*}{$\indicator{\neighbor{3}{t} = j}$} & \multirow{2}{*}{$\cdots$} & \multirow{2}{*}{$0$} \\ Cost $\tfrac12$ \\
  \textbf{Action} $4$ & \multirow{2}{*}{$\indicator{t = 1}$} & \multirow{2}{*}{$\cdots$} & \multirow{2}{*}{$\indicator{t = j}$} & \multirow{2}{*}{$\cdots$} & \multirow{2}{*}{$0$} \\ Cost $\tfrac12$ \\
  \textbf{Action} $5$ & \multirow{2}{*}{$0$} & \multirow{2}{*}{$\cdots$} & \multirow{2}{*}{$0$} & \multirow{2}{*}{$\cdots$} & \multirow{2}{*}{$1$} \\ Cost $0$ \\ \midrule
  % Minimize Number of Sets
  \multirow{2}{*}{Type $t \in [N+1, 2N]$} & \textbf{Outcome} $1$ & \multirow{2}{*}{$\cdots$} & \textbf{Outcome} $j \in [N]$ & \multirow{2}{*}{$\cdots$} & \textbf{Outcome} $N+1$ \\
                                          & Reward $1$           &                           & Reward $1$                   &                           & Reward $0$             \\ \midrule
  \textbf{Action} $1$ & \multirow{2}{*}{$0$} & \multirow{2}{*}{$\cdots$} & \multirow{2}{*}{$0$} & \multirow{2}{*}{$\cdots$} & \multirow{2}{*}{$1$} \\ Cost $\tfrac12$ \\
  \textbf{Action} $2$ & \multirow{2}{*}{$0$} & \multirow{2}{*}{$\cdots$} & \multirow{2}{*}{$0$} & \multirow{2}{*}{$\cdots$} & \multirow{2}{*}{$1$} \\ Cost $\tfrac12$ \\
  \textbf{Action} $3$ & \multirow{2}{*}{$0$} & \multirow{2}{*}{$\cdots$} & \multirow{2}{*}{$0$} & \multirow{2}{*}{$\cdots$} & \multirow{2}{*}{$1$} \\ Cost $\tfrac12$ \\
  \textbf{Action} $4$ & \multirow{2}{*}{$0$} & \multirow{2}{*}{$\cdots$} & \multirow{2}{*}{$0$} & \multirow{2}{*}{$\cdots$} & \multirow{2}{*}{$1$} \\ Cost $\tfrac12$ \\
  \textbf{Action} $5$ & \multirow{2}{*}{$\indicator{t = N + 1}$} & \multirow{2}{*}{$\cdots$} & \multirow{2}{*}{$\indicator{t = N + j}$} & \multirow{2}{*}{$\cdots$} & \multirow{2}{*}{$0$} \\ Cost $0$ \\ \midrule
  \bottomrule
\end{tabular}
\caption{Counterexample principal-agent problem $\PrincipalAgentProblem$ constructed from an instance of \DSet{}. The types $t \in [N]$ generate one-half unit of profit if their corresponding vertex $t$ is dominated, and the types $t \in [N+1, 2N]$ eliminate one-half unit of profit if their corresponding vertex $(t - N)$ is chosen to be in the dominating set.}
\label{tab:example}
\end{table}
